Bayes without Underfitting: Fully Correlated Deep Learning Posteriors via Alternating Projections

Bayesian deep learning all too often underfits so that the Bayesian prediction is less accurate than a simple point estimate. Uncertainty quantification then comes at the cost of accuracy. For linearized models, the null space of the generalized Gauss-Newton matrix corresponds to parameters that preserve the training predictions of the point estimate. We propose to build Bayesian approximations in this null space, thereby guaranteeing that the Bayesian predictive does not underfit. We suggest a matrix-free algorithm for projecting onto this null space, which scales linearly with the number of parameters and quadratically with the number of output dimensions. We further propose an approximation that only scales linearly with parameters to make the method applicable to generative models. An extensive empirical evaluation shows that the approach scales to large models, including vision transformers with 28 million parameters.

==> old_stuff.tex <==

\section{Idea}
The core idea is to use the well-known logic equivalence: given two predicates $A$ and $B$ it hold
\begin{equation}
    A \textnormal{ and } B
    =
    \textnormal{not }
    \left(
    (\textnormal{not }A)
    \textnormal{ or }
    (\textnormal{not }B)
    \right)
\end{equation}
and specifically we want to apply it to projections. Given a matrix and its eigendecomposition $M=\sum_i \lambda_i v_iv_i^\top$ let its projection be defined as
\begin{equation}
    \mathcal{P}(M) = \sum_i \delta_{\lambda_i\not=0} v_iv_i^\top
\end{equation}
which has the same eigendecomposition of $M$ with the difference that the non-zero eigenvalues are set to 1.

Turns out that for positive semidefinite matrixes:
\begin{itemize}
    \item the projection over a sum of matrixes behave like an "and" statementent,
    \item the product of projections (to the power of $\infty$) behave like an "or" statement
    \item identity minus projection behave like a "not" statement
\end{itemize}
This implies that
\begin{equation}
    \mathcal{P}(M_1 \underbrace{+}_{\textnormal{and}} M_2)
    =
    \underbrace{\mathcal{I} - }_{\textnormal{not}}
    \lim_{T\rightarrow\infty}
    \left(
        (\underbrace{\mathcal{I} - }_{\textnormal{not}} \mathcal{P}(M_1))
        \underbrace{\cdot}_{\textnormal{or}}
        (\underbrace{\mathcal{I} - }_{\textnormal{not}} \mathcal{P}(M_2))
    \right)^T 
\end{equation}
and more generally that
\begin{equation}
    \mathcal{P}\left(\sum_n M_n\right)
    =
    \mathcal{I} - 
    \lim_{T\rightarrow\infty}
    \left(
        \prod_n 
        (\mathcal{I} - \mathcal{P}(M_n))
    \right)^T 
\end{equation}

\subsection{Deep Learning}
Given a neural network $f:\mathbb{R}^P\times\mathbb{R}^I\rightarrow\mathbb{R}^O$ and a parameter $\theta\in\mathbb{R}^P$, for any datapoint $x\in\mathbb{R}^I$ 
we can define the per-datum Jacobian as $\J_{\theta}(x) = \partial_{\theta} $ 
$f(\theta, x) \in \mathbb{R}^{O \times D}$. For a given collection of data $x_1,\ldots,x_N$, the Generalized Gauss Newton matrix is defined as
\begin{equation}
    GGN = \sum_n \J_{\theta}(x_n)^\top \J_{\theta}(x_n)
\end{equation}
and we can then compute the projection on the GGN as
\begin{equation}
    \mathcal{P}(GGN) = 
    \mathcal{I} - 
    \lim_{T\rightarrow\infty}
    \left(
        \prod_n 
        \left(
            \mathcal{I} - \mathcal{P}\Big(\J_{\theta}(x_n)^\top \J_{\theta}(x_n)\Big)
        \right)
    \right)^T 
\end{equation}
which doesn't seems very appealing until you notice that 
\begin{equation}
    \mathcal{P}\Big(\J_{\theta}(x_n)^\top \J_{\theta}(x_n)\Big)
    =
    \J_{\theta}(x_n)^\top 
    \left(
    \\J_{\theta}(x_n) \J_{\theta}(x_n)^\top
    \right)^{-1}
    \J_{\theta}(x_n)
\end{equation}
where the inversion happens on a small $O\times O$ matrix

% \subsubsection*{Acknowledgments}
% Use unnumbered third level headings for the acknowledgments. All
% acknowledgments, including those to funding agencies, go at the end of the paper.

\section{Alternative approach to explain the same thing}


\subsection{Deep Learning}
Ei what a coincidence if we set $M$ to be the Jacobian matrix of a neural network with respect to parameter, where now $n$ correspond to the product of dataset size and output dimensionality, then the square matrix $M^\top M \in\mathbb{R}^{p\times p}$ is called Generalized Gauss Newton and being able to project on its image would be actually cool.

